A Randomized Algorithm for Single-Source Shortest Path on Undirected Real-Weighted Graphs

In undirected graphs with real non-negative weights, we give a new randomized algorithm for the single-source shortest path (SSSP) problem with running time $O(m\sqrt{\log n \cdot \log\log n})$ in the comparison-addition model. This is the first algorithm to break the $O(m+n\log n)$ time bound for real-weighted sparse graphs by Dijkstra's algorithm with Fibonacci heaps. Previous undirected non-negative SSSP algorithms give time bound of $O(m\alpha(m,n)+\min\{n\log n, n\log\log r\})$ in comparison-addition model, where $\alpha$ is the inverse-Ackermann function and $r$ is the ratio of the maximum-to-minimum edge weight [Pettie & Ramachandran 2005], and linear time for integer edge weights in RAM model [Thorup 1999]. Note that there is a proposed complexity lower bound of $\Omega(m+\min\{n\log n, n\log\log r\})$ for hierarchy-based algorithms for undirected real-weighted SSSP [Pettie & Ramachandran 2005], but our algorithm does not obey the properties required for that lower bound. As a non-hierarchy-based approach, our algorithm shows great advantage with much simpler structure, and is much easier to implement.

==> algorithm-alternative.tex <==
\section{Main Algorithm}
\label{sec:algorithm}

In the following sections we assume that $G$ is connected, and each vertex in $G$ has degree no more than $3$. (There are $O(m)$ vertices and $O(m)$ edges in $G$, but we still use $O(\log n)$ which is equivalent to $O(\log m)$ where $n$ is the number of vertices in the original graph without degree constraints.)

%In the initialization state we sample a random subset of vertices $R$, and ``bundle'' each vertex to the closest $R$-vertex. By bundle we mean to bundle the process of a vertex, to the $R$ vertex it bundles to. Our algorithm works similarly as the original Dijkstra algorithm, however, only on vertices in $R$. We maintain a Fibonacci heap for vertices of $R$, and whenever a vertex $u\in R$ is popped, we handle all the vertices bundled to $u$. In this way, we only need the order of a subset of vertices, so it is possible to spend less time; and by the nature of bundle, that each vertex $v$ is bundled to the closest vertex in $R$, it is just about the right time to update $v$.

Our algorithm is based on original Dijkstra's algorithm \cite{Dij59}. Since the main bottleneck of Dijkstra's algorithm is the $O(\log n)$ time per every vertex extracted from the Fibonacci heap~\cite{FT87}, we only insert a subset $R \subseteq V$ of vertices into heap. Each remaining vertex $v\in V \setminus R$ is \emph{bundled} to its closest vertex in $R$. Throughout the algorithm, vertices are updated only when some vertex $u\in R$ is popped from the heap. Our algorithm consists of two stages: \emph{bundle construction} and \emph{bundle Dijkstra}, whose details will be introduced in Section \ref{sec:constructing-bundles} and \ref{sec:bundle-dijkstra} respectively.

To demonstrate the main idea of our algorithm, in this section we first give an algorithm that runs in expected $O(m\sqrt{\log n\cdot \log\log n})$ time but not ``with high probability''. In Section \ref{sec:improved-construction-of-bundles} we give an improved version of the bundle construction stage, leading to an algorithm that runs in $O(m\sqrt{\log n\cdot \log\log n})$ time with high probability. Both algorithms always give correct answers.

\subsection{Bundle Construction}
\label{sec:constructing-bundles}

A simple version of bundle construction work as follows ($k$ is a parameter to be determined later):
\begin{itemize}
    \item Independently sample each vertex $v\in V\setminus \{s\}$ with probability $\frac{1}{k}$ to form set $R$, then add $s$ into $R$.
    \item For each vertex $v \notin R$, run Dijkstra's algorithm started from $v$ until first vertex of $R$ is extracted from the heap, denoted by $\bundle(v)$. Therefore $\bundle(v)$ is one of the closest vertices in $R$ to $v$, i.e., $\bundle(v) \in \arg\min_{u\in R}\dis(u, v)$. We say that $v$ is \emph{bundled} to $\bundle(v)$.
    \item For each $u\in R$, let $\bundle(u) = u$, and $\Bundle(u) = \{v: u = \bundle(v)\}$ be the set of vertices bundled to $u$. By definition, $\{ \Bundle(u)\}_{u\in R}$ forms a partition of the vertex set $V$.
    \item For each vertex $v \notin R$, define $\Ball(v) = \{w\in V: \dis(v, w) < \dis(v, \bundle(v))\}$, that is, the set of vertices closer to $v$ than its bundled vertex $\bundle(v)$. In the previous Dijkstra's algorithm we also get values of $\dis(v, w)$ for all $w\in \Ball(v)\cup\{\bundle(v)\}$.
\end{itemize}

\paragraph{Time Analysis of Bundle Construction.} For each vertex $v\notin R$, without loss of generality we assume its Dijkstra's algorithm breaks tie in a deterministic way. Therefore, the order of vertices extracted from heap is fixed.

We can see $\mathbb{E}[|R|]=O(m/k)$. For each vertex $v\notin R$, let $S_v$ be the set of vertices extracted before its Dijkstra's algorithm stops, then $\Ball(v) \subsetneq S_v$. By definition of $R$, $\abs{S_v}$ follows geometric distribution with success probability $\frac{1}{k}$, thus $\mathbb{E}[\abs{S_v}]=k$ and $\mathbb{E}[\abs{\Ball(v)}] \leq k$.
By constant degree property, the number of vertices ever added into the heap is also $O(\abs{S_v})$, so the total time of the bundle construction is $O(\sum_{v\in V\setminus R} \mathbb{E}[\abs{S_v}\log \abs{S_v}])=O(mk\log k)$ in expectation.

\begin{remark}
One may notice that $x\log x$ is a convex function so that $\mathbb{E}[\abs{S_v}\log \abs{S_v}] = O(k\log k)$ does not trivially hold. We present a simple proof here: (by geometric distribution $\mathbb{E}[\abs{S_v}^2] = 2k^2 - k$)
\begin{align*}
\mathbb{E}[\abs{S_v}\log \abs{S_v}] &= \sum_{n = 1}^{\infty} \frac{1}{k}\left(1 - \frac{1}{k}\right)^{n-1}\cdot n\log n\\
&\leq \sum_{n\leq k^2} \frac{1}{k}\left(1 - \frac{1}{k}\right)^{n-1}\cdot n\log n + \sum_{n > k^2} \frac{1}{k}\left(1 - \frac{1}{k}\right)^{n-1}\cdot n^2\\
&\leq 2\log k \sum_{n\leq k^2} \frac{1}{k}\left(1-\frac{1}{k}\right)^{n-1}\cdot n + \sum_{n = 1}^{\infty}\frac{1}{k}\left(1 - \frac{1}{k}\right)^{k^2 + (n - 1)} (n + k^2)^2\\
&\leq 2\log k \cdot \mathbb{E}[\abs{S_v}] + \left(1 - \frac{1}{k}\right)^{k^2} \cdot \mathbb{E}[(\abs{S_v}+k^2)^2]\\
&\leq 2 k \log k + e^{-k} \cdot O(k^4) = O(k\log k).
\end{align*}

\end{remark}

%we sample $R$ from $V$ with probability $\frac{1}{k}$. For each vertex $v\in V$, denote 
%$\bundle(v) = \arg\min_{u\in R}\dis(u, v)$ to be the closest vertex of $R$ to $v$ and break tie arbitrarily; define $\Ball(v) = \{u\in V: \dis(v, u) < \dis(v, \bundle(v))\}$, that is the set of vertices closer to $v$ than $\bundle(v)$. And for each $u\in R$, define $\Bundle(u) = \{v: u = \bundle(v)\}$, that is the set of vertices bundled to $u$, and note that $u$ is bundled to itself. Therefore, $\{\Bundle(u)\}_{u\in R}$ forms a partition of the vertex set $V$.

%let k = \sqrt{\log n/\log \log n}
%then mk\log k + m\log n/k = m\sqrt{\log n\log\log n}.
\subsection{Bundle Dijkstra}
\label{sec:bundle-dijkstra}

In this section, we state our intuition of bundle Dijkstra before presenting the algorithm.

\paragraph{Intuition.} Given the set $R \subseteq V$ and that each vertex $v \in V \setminus R$ is bundled to its closest vertex in $R$, the algorithm should work similarly to Dijkstra's algorithm on vertices in $R$, and satisfy the following propositions:

\begin{enumerate}
    \item Vertices in $R$ are extracted from the heap in increasing order of $\dis(s,\cdot)$.
    
    \item When extracting an vertex $u\in R$ from the heap, its distance $\dis(s,u)$ is already found.
    
    \item After $u\in R$ extracted from the heap, the algorithm finds $\dis(s,x)$ for any $x \in \Bundle(u)$.
\end{enumerate}

The order of extracting $R$-vertices allows the algorithm to find $\dis(s, u)$ before $u \in R$ is extracted from heap. This is because, for any vertex $u\in R$, the shortest path from $s$ to $u$ only contains vertices $y$ with $\dis(s, \bundle(y)) \leq \dis(s, u)$, or more generally,
\begin{lemma}\label{lemma:R-vertex}
    For any vertex $u\in R$ and any path $P$ from $s$ to $u$, if $P$ goes through vertex $y$, $\dis(s,\bundle(y))$ is at most the length of $P$.
\end{lemma}
\begin{proof}
    $\dis(s, y)$ is at most the length of subpath of $P$ from $s$ to $y$. By definition of $\bundle(y)$, $\dis(y, \bundle(y))$ is at most the length of subpath of $P$ from $y$ to $u$. Concatenating two subpaths together, $\dis(s, \bundle(y)) \leq \dis(s, y) + \dis(y, \bundle(y))$ is at most the length of $P$.
\end{proof}

To update other $R$-vertices from vertices in $\Bundle(u)$, after $\dis(s,x)$ found for all $x\in \Bundle(u)$, $x$ should update its neighbors $y\in N(x)$ and $y$ should update its bundled vertex $\bundle(y)$.

The remaining part is to find $\dis(s,v)$ for any $v\in \Bundle(u)$ after $u$ is extracted. First is to update $v$ from $u$. If $\dis(s,v)<\dis(s,u)+\dis(u,v)$, Consider the shortest path $P$ from $s$ to $v$.
If $P$ only pass through vertices $x$ whose bundled vertex $\bundle(x)$ is extracted before $u$, previous updates is sufficient to find $\dis(s, v)$. Otherwise, let $x$ be last vertex on $P$ such that $\bundle(x)$ is extracted before $u$, and $y$ be the next one after $x$.
For this case, we have the following lemma:
\begin{lemma}\label{lemma:other}
    On the shortest path from $y$ to $v$ there are two adjacent vertices $z_1,z_2$ such that $z_1\in\Ball(y)\cup\{y\}$ and $z_2\in\Ball(v)\cup\{v\}$.
\end{lemma}

\begin{proof}
    We have $\dis(y,v)=\dis(s,v)-\dis(s,y)$ and $\dis(s,v)<\dis(s,u)+\dis(u,v)$. By triangle inequality, $\dis(s,y)\geq \dis(s,\bundle(y))-\dis(y,\bundle(y))$, and by $\dis(s,\bundle(y))\geq \dis(s,u)$,
    \begin{align*}
        \dis(y,v) < & ~ \dis(u,v) + \dis(y,\bundle(y))\\
        & ~ \dis(u,v)+\dis(y,\bundle(y))+\dis(s,u)-\dis(s,\bundle(y))\\
        \leq & ~ \dis(u,v)+\dis(y,\bundle(y))~.
    \end{align*}
    Let $z_1$ be the last vertex on the shortest path from $y$ to $v$ satisfying $\dis(y,z_1)<\dis(y,\bundle(y))$, so $z_1\in\Ball(y)$. Then $z_2$ will be the next vertex after $z_1$, so $\dis(y,z_2)\geq\dis(y,\bundle(y))$, and $\dis(z_2,v)<\dis(v,u)$, so $z_2\in\Ball(v)$. (If $\dis(y,\bundle(y))=0$ then $z_1=y$, and if $\dis(y,v)<\dis(y,\bundle(y))$ then $z_2=v$ and $z_1$ is the vertex before $v$.)
\end{proof}

After finding $z_1, z_2$, we may update $z_1$ through $y$ from $x$. Since $\bundle(x)$ is extracted before $u$, $\dis(s, z_1)$ is found before $u$ is extracted. Then after $u$ is extracted, we may update $v$ through $z_2$ from $z_1$ to find $\dis(s, v)$. 


\paragraph{Algorithm.} Based on aforementioned ideas, bundle Dijkstra work as follows, with pseudocode given in Algorithm~\ref{alg:bundle-Dijkstra}:

Initially we set $d(s)=0$ and $d(v)=+\infty$ for all other vertex $v$, and insert all vertices of $R$ into a Fibonacci heap~\cite{FT87}. Whenever we pop a vertex $u\in R$ from the heap, we update the distances by the following steps. (Relaxing a vertex $v$ by a value $D$ means that we update $d(v)$ by $\min\{d(v), D\}$)
\begin{enumerate}
    \item For every vertex $v$ bundled to $u$, we need to find the exact value of $\dis(s,v)$. First relax $v$ by $d(u)+\dis(u,v)$; then for every vertex $y\in\Ball(v)$, relax $v$ by $d(y)+\dis(y,v)$; and for every $z_2 \in \Ball(v)\cup\{v\}$ and $z_1\in N(z_2)$, relax $v$ by $d(z_1)+w_{z_1,z_2}+\dis(z_2,v)$. That is, we update $d(v)$ by its bundled vertex $u$, vertices in $\Ball(v)$, and vertices neighboring to $v$ and $\Ball(v)$.
    \item Then by the current value $d(v)$ for $v\in\Bundle(u)$, we update the vertices $y\in N(v)$ and vertices $z_1\in\Ball(y)$. That is, relaxing $y$ by $d(v)+w_{v,y}$ for all $y\in N(v)$ and then relaxing $z_1$ by $d(v)+w_{v,y}+\dis(y,z_1)$ for all $z_1\in\Ball(y)$.
    \item Whenever we update a vertex $x\notin R$, we also relax its bundled vertex $\bundle(x)$ by $d(x)+\dis(x,\bundle(x))$. (But later we will see this is only needed in Step 2 but not Step 1, since in Step 1 $v$ is bundled to $u$, but the distance $\dis(s,u)$ is already found when popping $u$ from the heap.)
\end{enumerate}

The following observation holds naturally from the algorithm.

\begin{observation}\label{obs:d-upper-bound}
    $d(v) \geq \dis(s, v)$ always holds for all $v \in V$.
\end{observation}

\paragraph{Time Analysis for Bundle Dijkstra.} For the bundle Dijkstra stage, only vertices in $R$ are inserted into heap, thus the extract-min operation only takes $O(\abs{R}\log n)$ time in total. Since every vertex $v\in V\setminus R$ only appear once in Step 1 and Step 2, and by constant degree property, every vertex appears constant times as the vertex $y\in N(v)$ in Step 2. So the time for Step 1, 2 and 3 is $O(\sum_{v\in V\setminus R}|\Ball(v)|)$. Thus, the time of the bundle Dijkstra stage is $O(|R|\cdot\log n+\sum_{v\in V\setminus R}\abs{\Ball(v)}) = O(\frac{m}{k}\log n + mk)$ in expectation.

Now, we can see that the expected total time of the two stages is $O(\frac{m}{k}\log n + mk\log k)$, which is minimized to $O(m\sqrt{\log n\cdot \log \log n})$ if we choose $k = \sqrt{\frac{\log n}{\log \log n}}$. We move to explain our main ideas of the correctness proof. A formal proof is given in Section~\ref{sec:correctness-analysis}.

\begin{algorithm}
    \caption{\textsc{BundleDijkstra}$(G,s)$}
    \label{alg:bundle-Dijkstra}
    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
    \SetKwProg{Func}{function}{:}{}
    \Input{A graph $G=(V,E,w)$ and starting vertex $s\in V$}
    \Output{Distance $d(v)$ from $s$ to $v$ for every vertex $v\in V$}
    
    \nl Construct Bundles as described in Section~\ref{sec:constructing-bundles}\;
    
    \nl Set label $d(s) \gets 0$ and $d(v) \gets +\infty$ for all $v \in V\setminus \{s\}$\;
    
    \nl Initialize Fibonacci heap $H$ with all vertices of $R$ and key $d(\cdot)$\;
    
    \nl \While{$H$ is not empty}{
 
    \nl 	$u \gets H$.\textsc{ExtractMin}$()$\; \label{line:bundle-Dijkstra-extractmin}
        
    \nl     \ForEach(\tcp*[f]{Step 1}){$v \in \Bundle(u)$} {
        
    \nl         \textsc{Relax}($v$, $d(u) + \dis(u, v)$)\;\label{line:bundle-Dijkstra:update-uv}  
            
    \nl         \ForEach{$y \in \Ball(v)$}{
    
    \nl             \textsc{Relax}($v$, $d(y) + \dis(y, v)$)\; \label{line:bundle-Dijkstra-update-yv}
            }

    \nl         \ForEach{$z_2 \in \Ball(v)\cup\{v\}$}{
    
    \nl             \ForEach{$z_1 \in N(z_2)$}{
    
    \nl                 \textsc{Relax}($v$, $d(z_1) + w_{z_1, z_2} + \dis(z_2, v)$)\; \label{line:bundle-Dijkstra:update-z1v}
                }
            }
        }
        
    \nl     \ForEach(\tcp*[f]{Step 2}){$x \in \Bundle(u)$}{
            
    \nl         \ForEach{$y \in N(x)$}{

    \nl             \textsc{Relax}($y$, $d(x) + w_{x, y}$)\;\label{line:bundle-Dijkstra:update-xy}
                
    \nl             \ForEach{$z_1 \in \Ball(y)$}{
                
    \nl                 \textsc{Relax}($z_1$, $d(x) + w_{x, y} + \dis(y, z_1)$)\; \label{line:bundle-Dijkstra:update-xz1}

                    % \ForEach{$w \in \Ball(z_1)$}{
                        
                    %     \textsc{Relax}($w$, $d(z_1) + w_{z_1, w}$)\; 
                        
                    % }
                }
            }
        }
    }

    \Func{\textsc{\textrm{Relax($v$, $D$)}}}{
         \If{$D < d(v)$}{
            $d(v)\gets D$\;
            \If{$v\in H$}{
                $H$.\textsc{DecreaseKey}($v$, $D$)}
            \ElseIf{$v\notin R$}{
                \textsc{Relax}($\bundle(v), d(v) + \dis(v, \bundle(v))$)\tcp*[f]{Step 3}
            }
        }
        
    }
\end{algorithm}

\subsection{Proof of Correctness}
\label{sec:correctness-analysis}

We give a formal proof based on the pseudocode of Algorithm~\ref{alg:bundle-Dijkstra}. Define $u_i\in R$ as the vertex extracted in the $i$-th iteration of while-loop in Algorithm \ref{alg:bundle-Dijkstra}. Our key lemma in the following shows the main property of the algorithm.

\begin{lemma}
    \label{lem:shortest-path-iteration}
     The following properties hold for any $i\geq 1$ in Bundle Dijkstra (Algorithm \ref{alg:bundle-Dijkstra}):
    \begin{enumerate}
        \item When $u_i$ is extracted from the heap, $d(u_i) = \dis(s, u_i)$ holds. \label{prop:du-correct-before} 
        
        \item After $i$-th iteration of the while-loop, $d(u) \geq d(u_i)$ for all $u \in R \backslash \set{u_j}_{j\leq i}$. \label{prop:heap-pop-increase}
        
        \item After Step 1 of $i$-th iteration of the while-loop, $d(v)=\dis(s,v)$ for any $v \in \Bundle(u_i)$. \label{prop:dv-correct}
    \end{enumerate}
    
\end{lemma}

\begin{proof}
    We shall prove the lemma by induction on $i$.
    
    The lemma holds for $i = 1$ since $d(s) = 0$ and $d(v) = \dis(s, v)$ for all $v \in \Bundle(s)$.
    
    Suppose the lemma holds for every $i \leq t-1$, consider the case $i=t$.
    
    \begin{enumerate}
        \item Consider the shortest path $P$ from $s$ to $u_t$. Let $x$ be the last vertex on $P$ such that $x\in \Bundle(u_j)$ for some $j < t$, and $y$ be the next one after $x$, hence $y \in \Bundle(u)$ for some $u \in R \backslash \set{u_\ell}_{\ell < t}$. By Property \ref{prop:dv-correct} of induction hypothesis $d(x) = \dis(s, x)$ after Step 1 of $j$-th iteration. After that the algorithm updates $d(y)$, and further $d(u)$ in line \ref{line:bundle-Dijkstra:update-xy} since $y \in N(x)$.
        \begin{figure}[ht]
            \centering
            \begin{tikzpicture}
                \tikzstyle{mycircle}=[circle, minimum size = 6mm]
                \node [mycircle, draw, label=center:$s$] (s) at (-1.5, 0) {};
                \node [mycircle, draw, label=center:$x$] (x) at (0.5, 0) {};
                \node [mycircle, draw, label=center:$y$] (y) at (2, 0) {};
                \node [mycircle, draw, label=center:$u_j$] (uj) at (0.5, 1.5) {};
                \node [mycircle, draw, label=center:$u$] (u) at (2, 1.5) {};
                \node [mycircle, draw, label=center:$u_t$] (ut) at (4, 0) {};
                \draw [-latex, dashed] (s) .. controls (-0.75, 0.3) and (-0.25, -0.3) .. (x);
                \draw (x) -- (y);
                \draw [ultra thick] (x) -- (uj);
                \draw [ultra thick] (y) -- (u);
                \draw [-latex, dashed] (y) .. controls (2.75, 0.3) and (3.25, -0.3) .. (ut);
            \end{tikzpicture}
            \caption{Illustration of the shortest path from $s$ to $u_t$.}
        \end{figure}
        
        Therefore after $(t-1)$-th iteration $d(y) = \dis(s, x) + \dis(x, y) = \dis(s, y)$ and $d(u) \leq \dis(s, y) + \dis(y, u)$. Further:
        \begin{align*}
            d(u) \leq ~ & \dis(s, y) + \dis(y, u) \\
            \leq ~ &\dis(s, y) + \dis(y, u_t) \tag{$\bundle(y) = u$}\\
            = ~ &\dis(s, u_t) \tag{$y$ on shortest path}\\
            \leq ~ & d(u_t) \tag{Observation \ref{obs:d-upper-bound}}.
        \end{align*}

        On the other hand, the algorithm extracts $u_t$ from Fibonacci heap $H$ immediately after $(t-1)$-th iteration, thus $d(u_t) \leq d(u)$. So all the inequalities above should be equations, thus $d(u_t) = \dis(s, u_t)$.
        
        \item When executing line \ref{line:bundle-Dijkstra-extractmin} of $t$-th iteration, $d(u) \geq d(u_t)$ holds for every $u \in R \backslash \set{u_j}_{j\leq t}$ since $H$ is a Fibonacci heap. 
        Suppose $d(u) < d(u_t)$ for some $u \in R \backslash \set{u_j}_{j\leq t}$ after $t$-th iteration. The further updates on $d(u)$ must start from $d(x)$ for some $x \in \Bundle(u_t)$. For last such update, applying Lemma \ref{lemma:R-vertex} on this path from $s$ to $x$ then to $u$, we have:
        \begin{align*}
            d(u) \geq ~ & \dis(s, u_t) \tag{Lemma \ref{lemma:R-vertex}}\\
            = ~ & d(u_t), \tag{Property \ref{prop:du-correct-before}}
        \end{align*}
        leading to contradiction.
        
        \item By induction hypothesis it suffices to show that $d(v) = \dis(s, v)$ holds for all $v\in \Bundle(u_t)$.
        Suppose there exists a vertex $v\in \Bundle(u_t)$ such that $d(v)>\dis(s,v)$ after Step 1. Denote $P$ as the shortest path from $s$ to $v$. Let $x$ be the last vertex on $P$ such that $x\in \Bundle(u_j)$ for some $j < t$, and $y$ be the next one after $x$ on $P$, hence $y \in \Bundle(u)$ for some $u \in R \backslash \set{u_\ell}_{\ell < t}$. By Property \ref{prop:dv-correct} of induction hypothesis, $d(x) = \dis(s, x)$ after Step 1 of $j$-th iteration. Same as above we can show that $d(y) = \dis(s, x) + \dis(x, y) = \dis(s, y)$ and $d(u) \leq \dis(s, y) + \dis(y, u)$ (where $u=\bundle(y)$) before $t$-th iteration.
        We have:
        \begin{align*}
            \dis(s, y) \geq ~ & d(u) - \dis(y, u).\\
            \dis(s, v) < ~ & d(v) \tag{Assumption}\\
            \leq ~ & d(u_t) + \dis(u_t, v) \tag{$d(v)$ updated in Line \ref{line:bundle-Dijkstra:update-uv}}.
        \end{align*}
        
        On the other hand, $d(u) \geq d(u_t)$ after $t$-th iteration by Property \ref{prop:heap-pop-increase}. Since $d(u_t)$ doesn't change (Property \ref{prop:du-correct-before} and Observation \ref{obs:d-upper-bound}), $d(u)$ can only decrease in $t$-th iteration, so $d(u) \geq d(u_t)$ holds throughout $t$-th iteration. Hence:
        \begin{equation}
        \label{eq:hence-equation}
            \dis(y, v) = \dis(s, v) - \dis(s, y) < \dis(u_t, v) + \dis(y, u),
        \end{equation}
        while the equation holds since $y$ lies on the shortest path from $s$ to $v$.

        \begin{figure}[ht]
            \centering
            \begin{tikzpicture}
                \tikzstyle{mycircle}=[circle, minimum size = 6mm]
                \node [mycircle, draw, label=center:$s$] (s) at (-1.5, 0) {};
                \node [mycircle, draw, label=center:$x$] (x) at (0.5, 0) {};
                \node [mycircle, draw, label=center:$y$] (y) at (2, 0) {};
                \node [mycircle, draw, label=center:$u_j$] (uj) at (0.5, 1.5) {};
                \node [mycircle, draw, label=center:$u$] (u) at (2, 1.5) {};
                \node [mycircle, draw, label=center:$v$] (v) at (4, 0) {};
                \node [mycircle, draw, label=center:$u_t$] (ut) at (4, 1.5) {};
                \draw [-latex, dashed] (s) .. controls (-0.75, 0.3) and (-0.25, -0.3) .. (x);
                \draw (x) -- (y);
                \draw [ultra thick] (x) -- (uj);
                \draw [ultra thick] (y) -- (u);
                \draw [ultra thick] (v) -- (ut);
                \draw [-latex, dashed] (y) .. controls (2.75, 0.3) and (3.25, -0.3) .. (v);
                \draw (2, -1.1) arc(-90: 120: 1.1);
                \draw (4, -1.1) arc(270: 60: 1.1);
                
                \node [mycircle, draw, label=center:$x$] (x2) at (6, 0) {};
                \node [mycircle, draw, label=center:$y$] (y2) at (7.5, 0) {};
                \node [mycircle, draw, label=center:$z_1$] (z1) at (9.5, 0) {};
                \node [mycircle, draw, label=center:$z_2$] (z2) at (11, 0) {};
                \node [mycircle, draw, label=center:$v$] (v2) at (13, 0) {};
                
                \draw (x2) -- (y2);
                \draw [-latex, dashed] (y2) .. controls (8.25, 0.3) and (8.75, -0.3) .. (z1);
                \draw (z1) -- (z2);
                \draw [-latex, dashed] (z2) .. controls (11.75, 0.3) and (12.25, -0.3) .. (v2);
                \draw (9.5, 1.732) arc(60: -60: 2);
                \draw (11, 1.732) arc(120: 240: 2);
            \end{tikzpicture}
            \caption{Left: Illustration of the shortest path from $s$ to $v$ if $d(v) > \dis(s,v)$. Right: A closer look at path $x$ to $v$ if $\dis(y, v) \geq \dis(u_t, v)$.}
        \end{figure}
 
        Therefore there are two possible cases:
        \begin{itemize}
            \item $\dis(y, v) < \dis(u_t, v)$.
            
            In this case $y \in \Ball(v)$, so we can update $d(v)$ to $\dis(s,y)+\dis(y,v)$ on line \ref{line:bundle-Dijkstra-update-yv}, contradicting to $d(v)>\dis(s,v)$.
            
            \item $\dis(y, v) \geq \dis(u_t, v)$.
            
            First, by Inequality \eqref{eq:hence-equation}, $\dis(y, u) > \dis(y, v) - \dis(u_t, v) \geq 0$. Let $z_1$ be the last vertex on path $P$ with $\dis(y, z_1) < \dis(y, u)$, we have $z_1 \in \Ball(y)$.
            Let $z_2$ be the next vertex on the path, then $\dis(y, z_2)\geq \dis(y, u)$, so $\dis(z_2,v) = \dis(y, v) - \dis(y, z_2) \leq \dis(y, v) - \dis(y, u) < \dis(u_t,v)$, that is, $z_2\in \Ball(v)$.
            (If $z_2$ does not exist, then $z_1=v$.)
            
            By Property \ref{prop:dv-correct} of induction hypothesis, $d(x) = \dis(s, x)$ just after Step 1 of $j$-th iteration, so $d(z_1)$ is updated to $\dis(s, z_1)$ in line \ref{line:bundle-Dijkstra:update-xz1} of $j$-th iteration. Therefore $d(v)$ is updated to $\dis(s, v)$ in line \ref{line:bundle-Dijkstra:update-z1v} of $t$-th iteration (since $j < t$), contradicting the assumption.
        \end{itemize}

        Therefore $d(v)=\dis(s,v)$ for all $v \in \Bundle(u_t)$ after Step 1 of $t$-th iteration.
    \end{enumerate}

\end{proof}

\begin{remark}\label{rmk:lower-bound}
% How we break the sorting lower bound and the hierarchy property
% Traditional Dijkstra's algorithm computes, aside from shortest paths, a permutation $\pi_s:V \rightarrow V$ such that for any vertices $u,v\in V$, we find $\dis(s,u) > \dis(s,v) \Rightarrow \pi_s(u) > \pi_s(v)$. This is where sorting bottleneck comes from.
% \citet*{SV05} stated that, any SSSP algorithm for real-weighted graphs satisfying hierarchy property makes $\Omega(m + n\min\{\log\log r, \log n \})$ operations in the worst case, where $r$ is the ratio of the maximum to minimum edge length.
% \textbf{Hierarchy Property.} An SSSP algorithm on undirected graph with \emph{hierarchy property} computes, aside from shortest paths, a permutation $\pi_s:V \rightarrow V$ such that for any vertices $u,v\in V$, we find $\dis(s,u)\geq \dis(s,v) + \sep(u, v) \Rightarrow \pi_s(u) > \pi_s(v)$, where $\sep(u,v)$ is the longest edge on the MST path between $u$ and $v$.
% Our algorithm breaks these two bottlenecks since it has no restrictions on order of vertices bundled to same vertex $u\in R$.
Pettie and Ramachandran~\cite{SV05} proved that, any hierarchy-based SSSP algorithm on undirected graphs in comparison-addition model takes time at least $\Omega(m + \min\{n\log\log r, n\log n\})$, where $r$ is the ratio of the maximum-to-minimum edge weight. This bound becomes $\Omega(m+n\log n)$ when $r$ is exponentially large. Here the hierarchy-based algorithm is defined to generate a permutation $\pi_s$ satisfying \emph{hierarchy property:} $\dis(s, v)\geq \dis(s, u) + \sep(u, v) \Rightarrow \pi_{s}(u) < \pi_{s}(v)$, where $\sep(u, v)$ is the longest edge on the MST path between $u$ and $v$. The permutation $\pi_s$ is, though not defined to be, typically for the algorithms discussed in \cite{SV05}, the order that the algorithm visits the vertices. However, that is a worst-case lower bound, and our algorithm is randomized. Also the order that our algorithm visits the vertices \emph{does not} follow the hierarchy property: think of two vertices $x$ and $y$ are both connected to $u$ by edges $(x,u), (y,u)$ both with weight 1, and $x,y$ are both bundled to $u$. It is possible that $\sep(x,y)=1$ and $\dis(s, y)= \dis(s, x) + 2$ but we set no limit on the order we visit $x$ and $y$, that it is possible we visit $y$ before $x$. This explains why our algorithm can break this $\Omega(m + n\log n)$ lower bound in \cite{SV05}.

\end{remark}





%\subsection{Analysis of Running Time}
%\label{sec:running-time}

% The total time is $O\left(\frac{\abs{E}\log\abs{E}}{k} + \abs{E} k\right)$.

%The time for the initialization is $O(\sum_{v\in V}\abs{\Ball(v)} \log \abs{\Ball(v)})$, and the running time of algorithm \ref{alg:bundle-Dijkstra} is $O\left(\abs{R}\log n + \sum_{v\in V}\abs{\Ball(v)}\right)$.

%In expectation, $\abs{R} = \frac{m}{k}$ and $\Ball(v) = k$, so the total running time is $O(\frac{m\log n}{k} + mk\log k)$, and if we choose $k = \sqrt{\frac{\log n}{\log \log n}}$, the total running time is minimized and equal to $O(m\sqrt{\log n\cdot \log \log n})$.



==> conclusion.tex <==
\section{Conclusion}

In this paper we introduced our new randomized algorithm for the single-source shortest path(SSSP) problem with running time $O(m\sqrt{\log n\cdot \log\log n})$ on undirected graphs with non-negative real weights under the comparison-addition model. In section~\ref{sec:algorithm} we gave a form of our algorithm that runs in expected $O(m\sqrt{\log n\cdot \log\log n})$ time that always output the correct answer. The main idea is the bundle Dijkstra which bundles vertices to a smaller set $R$, so that we only need to sort the vertices in $R$, which enabled us to break the $\Omega(m + n\log n)$ lower bound. And in section~\ref{sec:constructing-bundles} we showed how to improve the construction of bundles to ensure the running time bounded by $O(m\sqrt{\log n\cdot \log\log n})$ with high probability.

Here are some possible future directions of our work:
\begin{itemize}
   \item Our algorithm benefits a lot from the constant degree property. Is it possible to work for a graph without this transformation, so that this result may not be limited to sparse graphs?
  \item Does this approach extend to directed graphs?
\end{itemize}

